A Hybrid Model of a Genetic Regulatory Network in Mammalian Sclera

Myopia in human and animals is caused by the axial elongation of the eye and is closely linked to the thinning of the sclera which supports the eye tissue. This thinning has been correlated with the overproduction of matrix metalloproteinase (MMP-2), an enzyme that degrades the collagen structure of the sclera. In this short paper, we propose a descriptive model of a regulatory network with hysteresis, which seems necessary for creating oscillatory behavior in the hybrid model between MMP-2, MT1-MMP and TIMP-2. Numerical results provide insight on the type of equilibria present in the system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{99}
\providecommand{\publicationstatus}{T. Dang and C. Piazza (Eds.): HSB 2013\\
EPTCS 125, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.125.8}{10.4204/EPTCS.125.8}}

